SmoothI: Smooth Rank Indicators for Differentiable IR Metrics

Information retrieval (IR) systems traditionally aim to maximize metrics built on rankings, such as precision or NDCG. However, the non-differentiability of the ranking operation prevents direct optimization of such metrics in state-of-the-art neural IR models, which rely entirely on the ability to compute meaningful gradients. To address this shortcoming, we propose SmoothI, a smooth approximation of rank indicators that serves as a basic building block to devise differentiable approximations of IR metrics. We further provide theoretical guarantees on SmoothI and derived approximations, showing in particular that the approximation errors decrease exponentially with an inverse temperature-like hyperparameter that controls the quality of the approximations. Extensive experiments conducted on four standard learning-to-rank datasets validate the efficacy of the listwise losses based on SmoothI, in comparison to previously proposed ones. Additional experiments with a vanilla BERT ranking model on a text-based IR task also confirm the benefits of our listwise approach.

==> tables/mq2007all.tex <==
\begin{tabular}{lllllllll}
 & P@1 & P@5 & P@10 & nDCG@1 & nDCG@5 & nDCG@10 & nDCG \\
SmoothP@1 & 0.469(0.009) & 0.408(0.007)$^{\ddagger}$ & 0.369(0.006)$^{\ddagger}$ & 0.424(0.009) & 0.424(0.010)$^{\ddagger}$ & 0.444(0.008)$^{\ddagger}$ & 0.602(0.006)$^{\ddagger}$ \\
SmoothP@5 & 0.470(0.013) & 0.408(0.009)$^{\ddagger}$ & 0.377(0.006)$^{\dagger}$ & 0.423(0.014) & 0.422(0.013)$^{\ddagger}$ & 0.449(0.010)$^{\ddagger}$ & 0.603(0.008)$^{\ddagger}$ & 0.450(0.009) \\
SmoothP@10 & 0.472(0.011) & 0.413(0.007)$^{\dagger}$ & 0.382(0.007) & 0.424(0.012) & 0.426(0.010)$^{\ddagger}$ & 0.455(0.009) & 0.604(0.006)$^{\ddagger}$ & 0.452(0.007) \\
SmoothNDCG@1 & 0.462(0.009) & 0.403(0.006)$^{\ddagger}$ & 0.363(0.006)$^{\ddagger}$ & 0.416(0.009) & 0.416(0.009)$^{\ddagger}$ & 0.437(0.006)$^{\ddagger}$ & 0.584(0.006)$^{\ddagger}$ & 0.411(0.008)$^{\ddagger}$ \\
SmoothNDCG@5 & 0.466(0.006) & 0.411(0.007)$^{\ddagger}$ & 0.375(0.007)$^{\ddagger}$ & 0.419(0.009) & 0.423(0.008)$^{\ddagger}$ & 0.447(0.007)$^{\ddagger}$ & 0.603(0.006)$^{\ddagger}$ & 0.450(0.007) \\
SmoothNDCG@10 & 0.471(0.011) & 0.416(0.006) & 0.380(0.006) & 0.423(0.011) & 0.428(0.009)$^{\dagger}$ & 0.454(0.009) & 0.601(0.007)$^{\ddagger}$ & 0.443(0.009) \\
SmoothNDCG & \textbf{0.488(0.007)} & \textbf{0.424(0.006)} & 0.384(0.006) & \textbf{0.441(0.010)} & \textbf{0.439(0.010)} & \textbf{0.461(0.008)} & \textbf{0.612(0.007)} & 0.461(0.007)
\end{tabular}


==> tables/mq2008all.tex <==
\begin{tabular}{lllllllll}
 & P@1 & P@5 & P@10 & nDCG@1 & nDCG@5 & nDCG@10 & nDCG & MAP \\
ListNet & 0.392(0.021)$^{\ddagger}$ & 0.318(0.016)$^{\ddagger}$ & 0.231(0.010)$^{\ddagger}$ & 0.339(0.017)$^{\ddagger}$ & 0.422(0.019)$^{\ddagger}$ & 0.468(0.019)$^{\ddagger}$ & 0.514(0.018)$^{\ddagger}$ & 0.428(0.016)$^{\ddagger}$ \\
ListMLE & 0.415(0.018)$^{\ddagger}$ & 0.337(0.017)$^{\ddagger}$ & 0.240(0.014)$^{\ddagger}$ & 0.365(0.018)$^{\dagger}$ & 0.445(0.019)$^{\ddagger}$ & 0.486(0.024)$^{\ddagger}$ & 0.526(0.021)$^{\ddagger}$ & 0.448(0.021)$^{\ddagger}$ \\
LambdaMARTP@1 & 0.431(0.015) & 0.339(0.017) & 0.270(0.013) & 0.358(0.012) & 0.447(0.019) & 0.495(0.019) & 0.532(0.018) & 0.467(0.017) \\
LambdaMARTP@5 & 0.450(0.022) & 0.347(0.014) & 0.274(0.012) & 0.376(0.017) & 0.458(0.017) & 0.502(0.019) & 0.537(0.019) & 0.476(0.018) \\
LambdaMARTP@10 & 0.432(0.024) & 0.344(0.015) & \textbf{0.275(0.012)} & 0.364(0.024) & 0.452(0.018) & 0.497(0.019) & 0.533(0.019) & 0.470(0.018) \\
LambdaMART@NDCG1 & 0.448(0.021) & 0.338(0.015) & 0.269(0.013) & 0.374(0.016) & 0.450(0.019) & 0.496(0.019) & 0.534(0.018) & 0.469(0.017) \\
LambdaMART@NDCG5 & 0.437(0.021) & 0.342(0.018) & 0.273(0.012) & 0.369(0.016) & 0.453(0.019) & 0.500(0.018) & 0.536(0.017) & 0.472(0.017) \\
LambdaMART@NDCG10 & 0.446(0.014) & 0.347(0.014) & 0.273(0.012) & 0.374(0.008) & 0.462(0.016) & 0.505(0.017) & 0.540(0.016) & 0.478(0.016) \\
LambdaMART@NDCG & 0.441(0.015) & 0.349(0.016) & \textbf{0.275(0.012)} & 0.368(0.011) & 0.461(0.016)$^{\dagger}$ & 0.505(0.017) & 0.538(0.017)$^{\dagger}$ & 0.477(0.016) \\
lambdaLossP@1 & 0.380(0.031)$^{\ddagger}$ & 0.309(0.017)$^{\ddagger}$ & 0.230(0.011)$^{\ddagger}$ & 0.336(0.028)$^{\ddagger}$ & 0.415(0.024)$^{\ddagger}$ & 0.469(0.023)$^{\ddagger}$ & 0.516(0.021)$^{\ddagger}$ & 0.436(0.022)$^{\ddagger}$ \\
lambdaLossP@5 & 0.366(0.015)$^{\ddagger}$ & 0.317(0.013)$^{\ddagger}$ & 0.231(0.010)$^{\ddagger}$ & 0.313(0.013)$^{\ddagger}$ & 0.411(0.017)$^{\ddagger}$ & 0.458(0.018)$^{\ddagger}$ & 0.504(0.018)$^{\ddagger}$ & 0.421(0.017)$^{\ddagger}$ \\
lambdaLossP@10 & 0.384(0.010)$^{\ddagger}$ & 0.318(0.013)$^{\ddagger}$ & 0.224(0.007)$^{\ddagger}$ & 0.335(0.010)$^{\ddagger}$ & 0.422(0.012)$^{\ddagger}$ & 0.458(0.011)$^{\ddagger}$ & 0.505(0.012)$^{\ddagger}$ & 0.415(0.007)$^{\ddagger}$ \\
lambdaLossNDCG@1 & 0.441(0.022) & 0.337(0.012)$^{\ddagger}$ & 0.242(0.010)$^{\ddagger}$ & 0.385(0.017) & 0.457(0.016)$^{\ddagger}$ & 0.500(0.016)$^{\dagger}$ & 0.540(0.017) & 0.467(0.014) \\
lambdaLossNDCG@5 & 0.435(0.019) & 0.336(0.013)$^{\ddagger}$ & 0.242(0.010)$^{\ddagger}$ & 0.384(0.017) & 0.452(0.017)$^{\ddagger}$ & 0.498(0.017)$^{\ddagger}$ & 0.537(0.017)$^{\dagger}$ & 0.462(0.015)$^{\ddagger}$ \\
lambdaLossNDCG@10 & 0.421(0.015) & 0.332(0.013)$^{\ddagger}$ & 0.241(0.009)$^{\ddagger}$ & 0.371(0.015) & 0.447(0.017)$^{\ddagger}$ & 0.493(0.018)$^{\ddagger}$ & 0.533(0.018)$^{\ddagger}$ & 0.456(0.016)$^{\ddagger}$ \\
lambdaLossNDCG & 0.421(0.031)$^{\dagger}$ & 0.334(0.013)$^{\ddagger}$ & 0.242(0.011)$^{\ddagger}$ & 0.368(0.026) & 0.449(0.019)$^{\ddagger}$ & 0.496(0.020)$^{\ddagger}$ & 0.535(0.020)$^{\ddagger}$ & 0.461(0.020)$^{\ddagger}$ \\
FSSNDCG & 0.430(0.012) & 0.332(0.014)$^{\ddagger}$ & 0.239(0.011)$^{\ddagger}$ & 0.371(0.010) & 0.450(0.014)$^{\ddagger}$ & 0.496(0.016)$^{\ddagger}$ & 0.537(0.015)$^{\dagger}$ & 0.461(0.012)$^{\ddagger}$ \\
SSOTNDCG & 0.431(0.014) & 0.342(0.014)$^{\dagger}$ & 0.245(0.011)$^{\ddagger}$ & 0.382(0.012) & 0.461(0.016)$^{\ddagger}$ & 0.504(0.017) & 0.542(0.017) & 0.470(0.014) \\
NSNDCG & 0.350(0.022)$^{\ddagger}$ & 0.293(0.014)$^{\ddagger}$ & 0.228(0.010)$^{\ddagger}$ & 0.304(0.016)$^{\ddagger}$ & 0.387(0.018)$^{\ddagger}$ & 0.448(0.017)$^{\ddagger}$ & 0.497(0.017)$^{\ddagger}$ & 0.402(0.014)$^{\ddagger}$ \\
ApproxP@1 & 0.443(0.026) & 0.349(0.013) & 0.246(0.010)$^{\ddagger}$ & 0.393(0.022) & 0.470(0.016) & 0.508(0.018) & 0.546(0.019) & 0.474(0.017) \\
ApproxP@5 & 0.448(0.023) & 0.343(0.016) & 0.246(0.012)$^{\ddagger}$ & 0.393(0.022) & 0.466(0.021) & 0.509(0.020) & 0.547(0.020) & 0.477(0.019) \\
ApproxP@10 & 0.454(0.020) & 0.344(0.016) & 0.245(0.011)$^{\ddagger}$ & 0.396(0.018) & 0.465(0.018) & 0.508(0.019) & 0.546(0.019) & 0.474(0.017) \\
ApproxNDCG@1 & 0.448(0.021) & 0.348(0.015) & 0.247(0.012)$^{\ddagger}$ & 0.393(0.020) & 0.471(0.017) & 0.511(0.019) & 0.547(0.018) & 0.476(0.016) \\
ApproxNDCG@5 & 0.445(0.020) & 0.346(0.014) & 0.247(0.011)$^{\ddagger}$ & 0.391(0.017) & 0.467(0.016) & 0.509(0.019) & 0.546(0.018) & 0.475(0.016) \\
ApproxNDCG@10 & 0.448(0.022) & 0.342(0.014) & 0.246(0.011)$^{\ddagger}$ & 0.395(0.021) & 0.464(0.019) & 0.509(0.019) & 0.546(0.019) & 0.474(0.017) \\
ApproxNDCG & 0.457(0.023) & 0.344(0.015) & 0.247(0.012)$^{\ddagger}$ & 0.401(0.020) & 0.468(0.017) & 0.513(0.020) & 0.549(0.019) & 0.478(0.018) \\
SmoothP@1 & 0.450(0.015) & 0.339(0.014)$^{\ddagger}$ & 0.243(0.011)$^{\ddagger}$ & 0.395(0.014) & 0.462(0.015) & 0.504(0.017) & 0.544(0.017) & 0.469(0.014) \\
SmoothP@5 & 0.443(0.015) & 0.342(0.015) & 0.245(0.011)$^{\ddagger}$ & 0.390(0.013) & 0.461(0.016)$^{\dagger}$ & 0.505(0.017) & 0.542(0.017) & 0.470(0.015) \\
SmoothP@10 & 0.449(0.018) & 0.347(0.014) & 0.248(0.012)$^{\ddagger}$ & 0.395(0.016) & 0.470(0.018) & 0.512(0.019) & 0.548(0.018) & 0.477(0.017) \\
SmoothNDCG@1 & 0.429(0.025) & 0.331(0.015)$^{\ddagger}$ & 0.238(0.012)$^{\ddagger}$ & 0.371(0.023) & 0.447(0.017)$^{\ddagger}$ & 0.489(0.019)$^{\ddagger}$ & 0.530(0.019)$^{\ddagger}$ & 0.453(0.017)$^{\ddagger}$ \\
SmoothNDCG@5 & 0.448(0.020) & 0.349(0.014) & 0.248(0.011)$^{\ddagger}$ & 0.391(0.019) & 0.469(0.017) & 0.509(0.018) & 0.546(0.018) & 0.474(0.015) \\
SmoothNDCG@10 & 0.457(0.022) & 0.350(0.015) & 0.248(0.010)$^{\ddagger}$ & \textbf{0.402(0.020)} & 0.472(0.019) & 0.513(0.019) & 0.549(0.019) & 0.479(0.017) \\
SmoothNDCG & \textbf{0.459(0.021)} & \textbf{0.353(0.015)} & 0.249(0.011)$^{\ddagger}$ & \textbf{0.402(0.018)} & \textbf{0.477(0.019)} & \textbf{0.514(0.019)} & \textbf{0.550(0.019)} & \textbf{0.481(0.018)}
\end{tabular}

==> tables/yltrall.tex <==
\begin{tabular}{lllllllll}
 & P@1 & P@5 & P@10 & nDCG@1 & nDCG@5 & nDCG@10 & nDCG & MAP \\
ListNet & 0.858(0.002)$^{\ddagger}$ & 0.814(0.001)$^{\ddagger}$ & 0.744(0.001)$^{\ddagger}$ & 0.726(0.001)$^{\ddagger}$ & 0.741(0.002)$^{\ddagger}$ & 0.777(0.001)$^{\ddagger}$ & 0.857(0.001)$^{\ddagger}$ & 0.846(0.001)$^{\ddagger}$ \\
ListMLE & 0.874(0.001)$^{\ddagger}$ & 0.829(0.001)$^{\ddagger}$ & 0.755(0.000)$^{\ddagger}$ & 0.724(0.005)$^{\ddagger}$ & 0.746(0.003) & \textbf{0.783(0.002)} & \textbf{0.859(0.002)} & 0.858(0.001)$^{\ddagger}$ \\
LambdaMARTP@1 & 0.875(0.000)$^{\ddagger}$ & 0.835(0.000)$^{\ddagger}$ & 0.810(0.000)$^{\ddagger}$ & 0.629(0.000)$^{\ddagger}$ & 0.658(0.000)$^{\ddagger}$ & 0.708(0.000)$^{\ddagger}$ & 0.806(0.000)$^{\ddagger}$ & 0.854(0.000)$^{\ddagger}$ \\
LambdaMARTP@5 & \textbf{0.882(0.000)} & 0.840(0.000)$^{\ddagger}$ & 0.814(0.000)$^{\ddagger}$ & 0.598(0.000)$^{\ddagger}$ & 0.654(0.000)$^{\ddagger}$ & 0.708(0.000)$^{\ddagger}$ & 0.802(0.000)$^{\ddagger}$ & 0.860(0.000)$^{\ddagger}$ \\
LambdaMARTP@10 & \textbf{0.882(0.000)} & \textbf{0.843(0.000)} & \textbf{0.816(0.000)} & 0.575(0.000)$^{\ddagger}$ & 0.645(0.000)$^{\ddagger}$ & 0.701(0.000)$^{\ddagger}$ & 0.797(0.000)$^{\ddagger}$ & \textbf{0.861(0.000)} \\
LambdaMART@NDCG1 & 0.871(0.000)$^{\ddagger}$ & 0.827(0.000)$^{\ddagger}$ & 0.803(0.000)$^{\ddagger}$ & 0.674(0.000)$^{\ddagger}$ & 0.689(0.000)$^{\ddagger}$ & 0.732(0.000)$^{\ddagger}$ & 0.823(0.000)$^{\ddagger}$ & 0.848(0.000)$^{\ddagger}$ \\
LambdaMART@NDCG5 & 0.873(0.000)$^{\ddagger}$ & 0.833(0.000)$^{\ddagger}$ & 0.807(0.000)$^{\ddagger}$ & 0.685(0.000)$^{\ddagger}$ & 0.704(0.000)$^{\ddagger}$ & 0.746(0.000)$^{\ddagger}$ & 0.830(0.000)$^{\ddagger}$ & 0.853(0.000)$^{\ddagger}$ \\
LambdaMART@NDCG10 & 0.874(0.000)$^{\ddagger}$ & 0.834(0.000)$^{\ddagger}$ & 0.808(0.000)$^{\ddagger}$ & 0.687(0.000)$^{\ddagger}$ & 0.705(0.000)$^{\ddagger}$ & 0.748(0.000)$^{\ddagger}$ & 0.831(0.000)$^{\ddagger}$ & 0.853(0.000)$^{\ddagger}$ \\
LambdaMART@NDCG & 0.874(0.000)$^{\ddagger}$ & 0.834(0.000)$^{\ddagger}$ & 0.809(0.000)$^{\ddagger}$ & 0.686(0.000)$^{\ddagger}$ & 0.705(0.000)$^{\ddagger}$ & 0.748(0.000)$^{\ddagger}$ & 0.831(0.000)$^{\ddagger}$ & 0.854(0.000)$^{\ddagger}$ \\
lambdaLossP@1 & 0.865(0.004)$^{\ddagger}$ & 0.816(0.006)$^{\ddagger}$ & 0.739(0.007)$^{\ddagger}$ & 0.667(0.011)$^{\ddagger}$ & 0.701(0.009)$^{\ddagger}$ & 0.739(0.010)$^{\ddagger}$ & 0.829(0.009)$^{\ddagger}$ & 0.826(0.015)$^{\ddagger}$ \\
lambdaLossP@5 & 0.868(0.004)$^{\ddagger}$ & 0.822(0.005)$^{\ddagger}$ & 0.747(0.006)$^{\ddagger}$ & 0.650(0.008)$^{\ddagger}$ & 0.701(0.009)$^{\ddagger}$ & 0.743(0.010)$^{\ddagger}$ & 0.832(0.008)$^{\ddagger}$ & 0.839(0.012)$^{\ddagger}$ \\
lambdaLossP@10 & 0.865(0.004)$^{\ddagger}$ & 0.818(0.006)$^{\ddagger}$ & 0.743(0.007)$^{\ddagger}$ & 0.636(0.008)$^{\ddagger}$ & 0.690(0.009)$^{\ddagger}$ & 0.734(0.011)$^{\ddagger}$ & 0.825(0.009)$^{\ddagger}$ & 0.830(0.017)$^{\ddagger}$ \\
lambdaLossNDCG@1 & 0.867(0.001)$^{\ddagger}$ & 0.818(0.001)$^{\ddagger}$ & 0.745(0.001)$^{\ddagger}$ & 0.730(0.003)$^{\dagger}$ & 0.737(0.002)$^{\ddagger}$ & 0.772(0.001)$^{\ddagger}$ & 0.854(0.001)$^{\ddagger}$ & 0.845(0.002)$^{\ddagger}$ \\
lambdaLossNDCG@5 & 0.865(0.002)$^{\ddagger}$ & 0.818(0.002)$^{\ddagger}$ & 0.745(0.002)$^{\ddagger}$ & 0.731(0.004) & 0.743(0.003)$^{\ddagger}$ & 0.775(0.003)$^{\ddagger}$ & 0.854(0.003)$^{\ddagger}$ & 0.843(0.005)$^{\ddagger}$ \\
lambdaLossNDCG@10 & 0.862(0.005)$^{\ddagger}$ & 0.813(0.006)$^{\ddagger}$ & 0.740(0.006)$^{\ddagger}$ & 0.730(0.005)$^{\dagger}$ & 0.739(0.007)$^{\ddagger}$ & 0.770(0.009)$^{\ddagger}$ & 0.850(0.008)$^{\ddagger}$ & 0.834(0.013)$^{\ddagger}$ \\
lambdaLossNDCG & 0.860(0.003)$^{\ddagger}$ & 0.812(0.004)$^{\ddagger}$ & 0.739(0.004)$^{\ddagger}$ & 0.726(0.002)$^{\ddagger}$ & 0.735(0.005)$^{\ddagger}$ & 0.766(0.007)$^{\ddagger}$ & 0.847(0.006)$^{\ddagger}$ & 0.832(0.011)$^{\ddagger}$ \\
FSSNDCG & 0.857(0.002)$^{\ddagger}$ & 0.812(0.001)$^{\ddagger}$ & 0.741(0.001)$^{\ddagger}$ & 0.724(0.001)$^{\ddagger}$ & 0.729(0.001)$^{\ddagger}$ & 0.765(0.001)$^{\ddagger}$ & 0.851(0.001)$^{\ddagger}$ & 0.842(0.001)$^{\ddagger}$ \\
SSOTNDCG & 0.846(0.026)$^{\ddagger}$ & 0.793(0.042)$^{\ddagger}$ & 0.719(0.047)$^{\ddagger}$ & 0.710(0.022)$^{\ddagger}$ & 0.719(0.040)$^{\ddagger}$ & 0.747(0.054)$^{\ddagger}$ & 0.842(0.026)$^{\ddagger}$ & 0.820(0.049)$^{\ddagger}$ \\
NSNDCG & 0.000(0.000)$^{\ddagger}$ & 0.000(0.000)$^{\ddagger}$ & 0.000(0.000)$^{\ddagger}$ & 0.000(0.000)$^{\ddagger}$ & 0.000(0.000)$^{\ddagger}$ & 0.000(0.000)$^{\ddagger}$ & 0.499(0.000)$^{\ddagger}$ & 0.356(0.000)$^{\ddagger}$ \\
ApproxP@1 & 0.869(0.002)$^{\ddagger}$ & 0.827(0.001)$^{\ddagger}$ & 0.754(0.000)$^{\ddagger}$ & 0.645(0.006)$^{\ddagger}$ & 0.703(0.004)$^{\ddagger}$ & 0.751(0.003)$^{\ddagger}$ & 0.840(0.002)$^{\ddagger}$ & 0.857(0.000)$^{\ddagger}$ \\
ApproxP@5 & 0.870(0.002)$^{\ddagger}$ & 0.827(0.001)$^{\ddagger}$ & 0.754(0.001)$^{\ddagger}$ & 0.645(0.012)$^{\ddagger}$ & 0.703(0.007)$^{\ddagger}$ & 0.750(0.005)$^{\ddagger}$ & 0.840(0.003)$^{\ddagger}$ & 0.857(0.001)$^{\ddagger}$ \\
ApproxP@10 & 0.869(0.002)$^{\ddagger}$ & 0.828(0.001)$^{\ddagger}$ & 0.754(0.000)$^{\ddagger}$ & 0.639(0.004)$^{\ddagger}$ & 0.701(0.002)$^{\ddagger}$ & 0.749(0.001)$^{\ddagger}$ & 0.839(0.001)$^{\ddagger}$ & 0.857(0.000)$^{\ddagger}$ \\
ApproxNDCG@1 & 0.863(0.003)$^{\ddagger}$ & 0.816(0.005)$^{\ddagger}$ & 0.733(0.008)$^{\ddagger}$ & 0.665(0.008)$^{\ddagger}$ & 0.703(0.006)$^{\ddagger}$ & 0.737(0.009)$^{\ddagger}$ & 0.833(0.005)$^{\ddagger}$ & 0.822(0.013)$^{\ddagger}$ \\
ApproxNDCG@5 & 0.869(0.001)$^{\ddagger}$ & 0.828(0.001)$^{\ddagger}$ & 0.752(0.000)$^{\ddagger}$ & 0.655(0.004)$^{\ddagger}$ & 0.708(0.002)$^{\ddagger}$ & 0.753(0.001)$^{\ddagger}$ & 0.841(0.001)$^{\ddagger}$ & 0.855(0.000)$^{\ddagger}$ \\
ApproxNDCG@10 & 0.868(0.002)$^{\ddagger}$ & 0.827(0.001)$^{\ddagger}$ & 0.754(0.000)$^{\ddagger}$ & 0.638(0.007)$^{\ddagger}$ & 0.700(0.004)$^{\ddagger}$ & 0.749(0.003)$^{\ddagger}$ & 0.838(0.002)$^{\ddagger}$ & 0.856(0.001)$^{\ddagger}$ \\
ApproxNDCG & 0.863(0.003)$^{\ddagger}$ & 0.818(0.001)$^{\ddagger}$ & 0.746(0.001)$^{\ddagger}$ & 0.731(0.002) & 0.745(0.001)$^{\ddagger}$ & 0.779(0.001)$^{\ddagger}$ & 0.858(0.001) & 0.848(0.001)$^{\ddagger}$ \\
SmoothP@1 & 0.866(0.001)$^{\ddagger}$ & 0.819(0.002)$^{\ddagger}$ & 0.744(0.001)$^{\ddagger}$ & 0.683(0.003)$^{\ddagger}$ & 0.712(0.001)$^{\ddagger}$ & 0.752(0.002)$^{\ddagger}$ & 0.842(0.001)$^{\ddagger}$ & 0.845(0.003)$^{\ddagger}$ \\
SmoothP@5 & 0.869(0.002)$^{\ddagger}$ & 0.825(0.003)$^{\ddagger}$ & 0.747(0.005)$^{\ddagger}$ & 0.665(0.005)$^{\ddagger}$ & 0.709(0.005)$^{\ddagger}$ & 0.750(0.006)$^{\ddagger}$ & 0.840(0.004)$^{\ddagger}$ & 0.845(0.009)$^{\ddagger}$ \\
SmoothP@10 & 0.868(0.001)$^{\ddagger}$ & 0.826(0.001)$^{\ddagger}$ & 0.750(0.001)$^{\ddagger}$ & 0.662(0.005)$^{\ddagger}$ & 0.709(0.002)$^{\ddagger}$ & 0.751(0.001)$^{\ddagger}$ & 0.841(0.001)$^{\ddagger}$ & 0.850(0.001)$^{\ddagger}$ \\
SmoothNDCG@1 & 0.858(0.001)$^{\ddagger}$ & 0.812(0.001)$^{\ddagger}$ & 0.740(0.001)$^{\ddagger}$ & 0.724(0.001)$^{\ddagger}$ & 0.726(0.001)$^{\ddagger}$ & 0.760(0.002)$^{\ddagger}$ & 0.849(0.001)$^{\ddagger}$ & 0.839(0.002)$^{\ddagger}$ \\
SmoothNDCG@5 & 0.859(0.003)$^{\ddagger}$ & 0.811(0.003)$^{\ddagger}$ & 0.737(0.004)$^{\ddagger}$ & 0.723(0.003)$^{\ddagger}$ & 0.731(0.004)$^{\ddagger}$ & 0.762(0.006)$^{\ddagger}$ & 0.849(0.003)$^{\ddagger}$ & 0.833(0.006)$^{\ddagger}$ \\
SmoothNDCG@10 & 0.854(0.003)$^{\ddagger}$ & 0.810(0.003)$^{\ddagger}$ & 0.738(0.003)$^{\ddagger}$ & 0.714(0.003)$^{\ddagger}$ & 0.726(0.004)$^{\ddagger}$ & 0.760(0.005)$^{\ddagger}$ & 0.848(0.003)$^{\ddagger}$ & 0.836(0.005)$^{\ddagger}$ \\
SmoothNDCG & 0.867(0.002)$^{\ddagger}$ & 0.821(0.000)$^{\ddagger}$ & 0.747(0.000)$^{\ddagger}$ & \textbf{0.735(0.003)} & \textbf{0.748(0.001)} & 0.780(0.001)$^{\ddagger}$ & 0.858(0.001) & 0.846(0.002)$^{\ddagger}$
\end{tabular}

